Efficiency through Uncertainty: Scalable Formal Synthesis for Stochastic Hybrid Systems

This work targets the development of an efficient abstraction method for formal analysis and control synthesis of discrete-time stochastic hybrid systems (SHS) with linear dynamics. The focus is on temporal logic specifications, both over finite and infinite time horizons. The framework constructs a finite abstraction as a class of uncertain Markov models known as interval Markov decision process (IMDP). Then, a strategy that maximizes the satisfaction probability of the given specification is synthesized over the IMDP and mapped to the underlying SHS. In contrast to existing formal approaches, which are by and large limited to finite-time properties and rely on conservative over-approximations, we show that the exact abstraction error can be computed as a solution of convex optimization problems and can be embedded into the IMDP abstraction. This is later used in the synthesis step over both finite- and infinite-horizon specifications, mitigating the known state-space explosion problem. Our experimental validation of the new approach compared to existing abstraction-based approaches shows: (i) significant (orders of magnitude) reduction of the abstraction error; (ii) marked speed-ups; and (iii) boosted scalability, allowing in particular to verify models with more than 10 continuous variables.

==> format_files/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/experiments.tex <==
% experiments

\begin{figure*}
  \centering
  \begin{subfigure}{.35\textwidth}
     \centering
     \includegraphics[width=1\linewidth]{LowerBouunddx05h011modeFlat.jpg}
     \caption{Verification, mode $a_1$}
     \label{fig:lower1mode}
  \end{subfigure}
  ~
  \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{LowerBouund_dx05h01_2modesynth_mode1_Flat.png}
    \caption{Synthesis, mode $a_1$}
    \label{fig:lower2mode_mode1}
  \end{subfigure}
  ~
  \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{LowerBouund_dx05h01_2modesynth_mode2_Flat.png}
    \caption{Synthesis, mode $a_2$}
    \label{fig:lower2mode_mode2}
  \end{subfigure}
  \caption{Verification and synthesis results for case studies 1 and 3.  The safe set $\safeSet$ is a rectangle, and the shades of gray correspond to the lower bound of the safety probability, where black and white correspond to values 0 and 1, respectively.   
  % (Figure \ref{fig:lower1mode}) $\Plow_q$ for all $q\in \Qimdp$ for the system in Eqn \eqref{ExperimentEqn}. (Figure \ref{fig:lower2mode}) $\Plow_q$ for all $q\in \Qimdp$ conditioned to the syntesized strategy $\str$ under the assumption that at time $0$ we are in mode $2$.
  }
  \label{Figure:ExperimentVerificationSyntesish0.1dx0.5}
\end{figure*}


We implemented our abstraction and synthesis algorithms in MATLAB and tested the performance of the framework on a set of case studies.  We first considered a stochastic process with a single mode to illustrate the efficacy and scalability of the approach in the formal analysis of SDEs (Case Study~1). Then, we analyzed the trade-off between space and time discretization parameters and their effects on the overall error (Case Study~2).  Finally, we considered a strategy synthesis problem on a two-mode switched stochastic process (Case Study~3).  

All the computations were performed on an Intel Dual Core i5 machine with 8 GB of RAM using a single thread program. Nevertheless, the implementation of the abstraction construction is highly parallelizable, allowing significant speedups.





\subsection{Case Study 1 - Verification}
\label{sec:VerifactionnCaseStudy}


We consider a stochastic process in the form of \eqref{eq:switched-dynamics} with $\U=\{a_1\}$,
% \begin{align}
% \label{ExperimentEqn}
%     d\pX(t)=F(a_1)\pX(t)+G(a_1)d\pW(t),
% \end{align}
\begin{equation*}
  F(a_1) =  
  \begin{pmatrix}
    -1 & 0 \\
    0    &  -0.5 \\
 \end{pmatrix},
 \quad
 G(a_1)= 
 % \begin{pmatrix}
 %    1 & 0 \\
 %    0 &  1 \\
 % \end{pmatrix},
 \Id,
\end{equation*}
and $\safeSet=[-8,8]\times[-8,8]$.
 % and $\pW$ is a Gaussian noise with zero mean and unitary variance.
% A system of SDEs is a particular case of switched diffusion, where there is just one possible strategy. We use this system to study how the different parameters influence the errors in the resulting \imdp abstraction.  More specifically, it is of interest to shed new lights about the relationship between space and time discretization parameters. 
% Then, we will complicate the model introducing a new possible (non-diagonal) mode, and show how the synthesized optimal strategy maximizes the safety and allow us to reduce errors.
 % We consider 
% the safe region $\safeSet=[-8,8]\times[-8,8]$. That is, an hyper-box centered in the origin.% Being the noise additive, for $\tau \to \infty$, the safety probability of $\pX$ being in $\safeSet$ for a duration $\tau$ will be always zero. 
  % We consider a duration $\tau=1$ 
% Being $G_1$ and $F_1$ diagonal we have that for any $h>0,q_i,q_j\subseteq \safeSet.
 % and the following property
  % $P_{\text{safe}}(\pX,\safeSet,\tau).$ That is, the probability that $\pX$ emains in $\safeSet$ during $[0,\tau]$. 
We are interested in the computation of the safety probability for every possible initial state of this model for the duration $\Tsafe = 1$.
In order to perform this analysis, we abstract the model to an \imdp.
% by discretizing time and space of $\pX$ . 
We use a sampling time of $\h=0.1$ and discretize $\safeSet$ in the transformed space induced by transformation function $\transfMatrix_{a_1}$, i.e., $\Post(\safeSet | \transfMatrix_{a_1})$, by a grid such that the size of each cell in the original space is $\dx=0.5$ per side.  This results in an \imdp abstraction with $|\Qimdp| = 1025$ states, and the discrete safety time steps $k_\Tsafe = 10$.
% , where $\transfMatrix_{a_1}=$. 
% The resulting \imdp abstraction had $|\Qimdp| = 1025$ states.  
% Call $\Qimdp$ the state space of the resulting \imdp abstraction.
We then run our \imdp (synthesis) algorithm to obtain the lower and upper bounds of the probability of safety, i.e., $\plow^{10}(q)$ and $\pup^{10}(q)$, for each possible initial state $q \in \Qimdp$. 
% That is, for $q \in \Qimdp$ we solved \eqref{eq:safety_bellman_lower} and \eqref{eq:safety_bellman_upper} and computed the interval $[\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q),\pup^{\lceil \frac{\Tsafe}{\h} \rceil}(q)].$

Figure \ref{fig:lower1mode} shows $\safeSet$ and the space discretization, where the lower bound of the probability of safety $\plow^{10}$ is marked as a shade of gray. The obtained upper bound probabilities were $\pup^{10}(q) \geq 0.97$ for all $\qimdp \in \Qimdp$.  It took a total of $175$ seconds to build the abstraction and compute the safety probability bounds.

In order to thoroughly analyze the error introduced by the discretization variables, we consider the local error term
  $$\err_q = \pup^{k_\Tsafe}(q) - \plow^{k_\Tsafe}(q),$$
and introduce the error metrics of $\errMed$, which is the median of $\err_q$ for all $q \in \Qimdp$, and $\errAve$, which is the average of $\err_q$ per unite volume given by
  $$\errAve=\frac{\sum_{q\in \Qimdp} \err_q \, \V_q}{\sum_{q\in \Qimdp} \V_q},$$
where $\V_q$ is the area (volume) of the region associated to state $q$.  For the chosen discretization variables $\h = 0.1$ and $\dx=0.5$, we obtain 
$\errMed=0.08 \quad \text{and} \quad \errAve=0.35.$
The smaller median error (than the average error) means that the majority of the cells have small errors $\err_q \leq 0.08$, and a small number of the cells have very large errors.  This can be explained by analyzing Figure \ref{fig:lower1mode}.  It is easy to observe that $\plow^{10}(q)\approx 0$ for the cells $q\in \Qimdp$ near $\partial\safeSet$, the boundary of $\safeSet$, i.e., $\err_q \approx 1$. 
In turn, for the cells $q \in Q$ that are not close to the boundary, $\err_q \approx 0$. 
This observation is aligned with the theory and the intuition as expressed in \eqref{eq:psafe_max_bound} and \eqref{eq:psafe_min_bound}.  That is, $\pX$ is a continuous-time diffusion process with a stable drift term $F(a_1)$ (the real eigenvalues are negative); hence, the process gets a strong pull towards the center, resulting in large upper bounds for safety probability in snapshots of $\h$ (discrete transition kernel), as suggested by \eqref{eq:psafe_max_bound}.  
% Thus, precisely computing the probability for the trajectories of $\pX$ to remain safe during $[0,\h]$ is easier if these do not start close to $\partial \safeSet.$
However, during this time, the probability of its continuous trajectory leaving $\safeSet$ is high due to the stochastic nature of the process if $\pX$ starts near $\partial \safeSet$, resulting in near-zero lower bound for the continuous transition kernel, i.e., $\alpha \approx 0$ in \eqref{eq:psafe_min_bound}.  
This suggests that the use of smaller cells near $\partial \safeSet$ can potentially reduce the spread of this effect (large error) to the nearby states, i.e., adaptive (non-uniform) gridding, as in \cite{SA13}.

%the safety probability computed on the \imdp abstraction with initial state $q$, where $[\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q)$ is the lower bound and $\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q)$ the upper bound of $P_{\text{safe}}(\pX,\safeSet,\tau)$ as computed on our \imdp abstraction. Then, for $q \in \Qimdp,$ we define the local error term
%  $\eta_q=|\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q) - [\pup^{\lceil \frac{\Tsafe}{\h} \rceil}(q)|$ and introduce the following error metrics $\epsilon_{avg}$ and $\epsilon_{me},$ where
%  $$\epsilon_{avq}=\frac{\sum_{q\in \Qimdp} |q|\eta_q     }{\sum_{q\in \Qimdp} |q| }  $$
%  and  $\epsilon_{me}$ is the median of $\eta_q$ for all $q \in \Qimdp.$ In the above, $|q|$ is the area of the region associated to state $q.$ %The required total time to build the abstraction and compute the required property is $175$ seconds. 
%  In Figure \ref{fig:lower1mode} we plot $\Plow_q$ for all $q\in \Qimdp.$
  
%   \begin{figure*}
%	\centering
%\begin{subfigure}{.3\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_lowerbound(1).png}
%     \caption{}
%     \label{fig:lower}
%   \end{subfigure}%
%\begin{subfigure}{.3\textwidth}
%  \centering
%  \includegraphics[width=1\linewidth]{exp_upperbound(1).png}
%  \caption{}
%  \label{fig:upper}
%\end{subfigure}
%\begin{subfigure}{.3\textwidth}
%  \centering
%  \includegraphics[width=1\linewidth]{err_profile_dt01.png}
%  \caption{}
%  \label{fig:error}
%\end{subfigure}
%\caption{ }
%\label{Figure:ExperimentSingleModeh0.1dx0.2}
%\end{figure*}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Case Study 2 - Analysis of Error Trade-off}
\label{sec:TradeoffTimeSpace}

In order to explore the trade-offs between the time and space discretization parameters and their effects on the overall error, we consider the same system as in Case Study 1 (Section \ref{sec:VerifactionnCaseStudy}) and perform safety analysis for the duration $\Tsafe=1$ with various values for $\h \in \set{0.05, \, 0.10,\, 0.15,\, 0.20,\, 0.25}$ and $\dx \in \set{0.20,\, 0.32,\, 0.40,\, 0.50,\, 0.64}$.
% , and for each of these values we discretize $\Post(\safeSet | \transfMatrix_{a_q})$ with a grid of cells of size $dx$ \ll{need to rescale according to $\transfMatrix_{a_1}$} and sample the time at a sampling time  $\h$. 
The obtained results are shown in Figure \ref{Figure:ExperimentSingleModeComparision}, 
% which  $\err_q$ $\forall q\in \Qimdp$ for each pair of values of $(\h,dx)$,
 % $\eta_q=|\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q) - [\pup^{\lceil \frac{\Tsafe}{\h} \rceil}(q)|$ 
illustrating the change in the distribution of $\err_q$ for the different values of $\h$ and $\dx$. 

Figure \ref{fig:fixeddx} is the box plot of $\err_q$, showing the distribution of $\err_q$ $\forall q \in \Qimdp$ for each pair $(\dx,\h)$ along with $\errMed$ (indicated with a red line) and $\errAve$ (indicated with a black star).  A general observation is that, by decreasing $\dx$, the distribution of the error becomes narrower and its average value decreases.
In Figure \ref{fig:fixeddt}, we plot $\errAve$ as a function of $\dx$ and $\h$. For each $\h$, $\errAve$ tends to decrease linearly with $\dx$. This is intuitive because a smaller $\dx$ means 
% a greater number of states in the resulting \imdp abstraction.
a smaller error due to space discretization for the same $\h$.
However, if we fix $\dx$ and consider different values of $\h$, we have a substantially different behavior: the error curve becomes parabolic. That is, for each $\dx$, there is an optimal value of $\h$ that minimizes $\errAve$, and this value of $\h$ is not necessarily the smallest one. This is due to the fact that, as discussed in Section \ref{sec:correctcomplete}, decreasing $\h$ causes a smaller variance in the discrete transition kernel, which means smaller cells are required to obtain a smaller overall error.  Moreover, the smaller the $\dx$ is, the smaller the optimal value of $\h$ becomes.  This means that, for a given finite $\dx$, if $\h$ is chosen to be too small,  some of the dynamics of the system may not be appropriately reflected in the abstraction, hence resulting in large errors.

\begin{figure*}
	\centering
  \begin{subfigure}{.49\textwidth}
     \centering
     \includegraphics[width=1\linewidth]{err_dist_fixed_dx_labeledaxis.png}
     \caption{}
     \label{fig:fixeddx}
  \end{subfigure}
  ~
  \begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{ave_err_bar3_labeledaxis.png}
  \caption{}
  \label{fig:fixeddt}
  \end{subfigure}
  \caption{Error distribution for the process in Case Study 2 with different values of $\h$ and $\dx$. (a) Box plot of $\err_q$ (blue boxes), $\errMed$ (red lines), and $\errAve$ (black stars). (b) 3-D plot of $\errAve$ as a function of $\h$ and $\dx$.  
  % (Figure \ref{fig:fixeddx}) For different values of $\dx$ we plot interquartile range, minimum and maximum of $\eta_q$, $\epsilon_{avg}$ (star), $\epsilon_{me}$ (red bar) at different values of $\h$.(Figure \ref{fig:fixeddt}) Plot of $\epsilon_{avg}$ for differfent values of $\h$ and $\dx$.  
  }
  \label{Figure:ExperimentSingleModeComparision}
\end{figure*}%



%The total error plotted in Figures \ref{fig:fixeddt} and \ref{fig:fixeddx} is due to two components: time discretization and space discretization.  For each $dx$ decreasing $\h$ the space discretization error increases becoming comparable with the total error.
%This is intuitive as it means that if using a discrete time model to model a continuous time system, then the sampling time must be small enough such that the probability of events happening between two sampling times becomes negligible. 

This case study shows that the choice of values for discretization parameters $\h$ and $\dx$ in order to obtain a desired overall error is not trivial.  One possible approach in tuning these parameters is to adapt a refinement technique to iteratively refine $\h$ and $\dx$ to arrive at the desired overall error value.  The proposed framework enables such an approach due to the low computation cost of abstraction and synthesis algorithms.
Another approach is to obtain a conservative approximation of the optimal value of $\dx$ for a given $\h$ before performing the computations, as shown in \cite{laurenti2017reachability}. However, since such approaches tend to be very conservative compared to our approach, this results in a very small $\dx$ to guarantee a given overall error, leading to state explosion. 

%. In fact, the error estimated in \cite{laurenti2017reachability} is global for all the states of the safe set. This leads to a very small $\dx$ to guarantee a given error. Thus, leading to the state space explosion problem. 

% value of the error orders of magnitude greater compared to the presented approach. 
% In fact, when $\h$ is small the Lipschitz constant of the discrete tranistion kernels increases. This leads to  to the state space explosion problem for existing methods \cite{esmaeil2013adaptive}. Our approach, being exact and not using over-approximation of the discrete transition kernel, mitigate such a problem. 


% Over approximation of the optimal value of $\h$ for a given $dx$ can be obtained before performing the computation, using a global error estimation of the error as shown in \cite{laurenti2017reachability}. However, such approaches tend to be very conservative, leading to a value of the error order of magnitude greater compared to our approach. In fact, when $\h$ is small the Lipschitz constant of the discrete tranistion kernels increases. This leads to  to the state space explosion problem for existing mehtods \cite{esmaeil2013adaptive}. Our approach, being exact and not using over-approximation of the discrete transition kernel, mitigate such a problem. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Case Study 3 - Switching Strategy Synthesis}
\label{sec:synthesisCaseStudy}

We add a second mode $a_2$ to the the process in Case Study 1 in Section \ref{sec:VerifactionnCaseStudy}, i.e., $\U = \set{a_1,a_2}$, where 
\begin{equation*}
  F(a_2)= 
  \begin{pmatrix}
    -0.5 & 0.1 \\
    0 &  -1 \\
  \end{pmatrix},  
  \quad
  G(a_2)= 
  % \begin{pmatrix}
  %   1 & 0 \\
  %   0 &  1 \\
  % \end{pmatrix}
  \Id.
\end{equation*}
% Thus, in the resulting switched stochastic systems we have $\U=\{a_1,a_2 \}$. 
We are interested in synthesizing a switching strategy that maximizes the probability of safety at every possible initial state with the duration of $\Tsafe = 1$ for the same $\safeSet$ as in Case Study 1.
In abstraction, we again use a sampling time $\h=0.1$. For space discretization, 
% for mode $a_1$, we consider a uniform grid over $\Post(\safeSet|\transfMatrix_{a_1})$ of cells of size $\dx=0.5$. For mode $a_2$ we discretize $\Post(\safeSet | \transfMatrix_{a_2})$ with a non-uniform grid composed of $1819$ states.
we use an adaptive grid such that the resulted cells have the maximum and minimum cells sizes of $\dx_{\max} = 0.5$ and $\dx_{\min} = 0.1$ in the original space.  
% Our adaptive grid algorithm discretizes $\Post(\safeSet|\transfMatrix_{a_i})$ for $i \in \set{1,2}$ by the maximum-sized cells where possible and minimum-sized cells where maximum-sized cells are not possible, which typically happens near $\partial \safeSet$. 
Our adaptive grid algorithm first over-approximates $\Post(\safeSet|\transfMatrix_{a_i})$ for $i \in \set{1,2}$ by using a uniform grid with the allowed maximum-sized cells.  Then, it refines the cells that are partly unsafe up to the resolution of the minimum-sized cells to under-approximate the safe set.
Figures \ref{fig:lower2mode_mode1} and \ref{fig:lower2mode_mode2} show the discretization of modes $a_1$ and $a_2$, respectively.  
Note that, in mode $a_2$, the cells are rotated which indicate that the transformation function $\transfMatrix_{a_2}$ includes a rotation in addition to translation.  The \imdp has a total of $|\Qimdp| = 2947$ states with $|\Qimdp^{a_1}| = 1024$, $|\Qimdp^{a_1}| = 1922$, and one $q_\unsafe$.  The total abstraction took 54 minutes.

% We solve \eqref{eq:safety_bellman_lower} and \eqref{eq:safety_bellman_upper} to syntesize a robust strategy $\str^*.$
  % For each $q \in \Qimdp$ we compute the resulting safety probability interval $[\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q)_{\str^*},\pup^{\lceil \frac{\Tsafe}{\h} \rceil}(q)_{\str^*}].$

We then run our synthesis algorithm to obtain the robust strategy $\str^*$ with its corresponding safety probability bounds $\plow^{10}_{\str^*}(q)$ and $\pup^{10}_{\str^*}(q)$ for all $q \in \Qimdp$.
In Figures \ref{fig:lower2mode_mode1} and \ref{fig:lower2mode_mode2} the lower bounds $\plow^{10}_{\str^*}$ are shown as shades of gray.  The upper bounds were $\pup^{10}_{\str^*}(q) \geq 0.93$ $\forall q\in \Qimdp$.  The synthesis computation took 15 seconds.

Call $\bar \str$ the strategy that always picks action $a_1$.  This strategy gives rise to the results obtained in Case Study 1 and presented in Figure \ref{fig:lower1mode}. Comparing it with the results of the strategy $\str^*$ in Figure \ref{fig:lower2mode_mode1}, it becomes evident that $\str^*$ improves the safety probability bounds, especially for the states near the top and bottom sides of $\safeSet$.  This means that $\str^*$ takes advantage of the drift in mode $a_2$ to keep the process safe in those sections of $\safeSet$.  More precisely, the median and average errors obtained for mode $a_1$ under $\str^*$ are $\errMed = 0.01$ and $\errAve = 0.28$, which show a reduction from the errors under $\bar\str$ where $\errMed = 0.08$ and $\errAve = 0.35$.


%it is possible to see how for all $q \in \ma$
%$$

%For $q\in\Qimdp$, we say that $q$ is safe with probability $p$ if $[\plow^{\lceil \frac{\Tsafe}{\h} \rceil}(q)_{\str}>p$. Comparing Figure \ref{fig:lower2mode} with Figure \ref{fig:lower1mode} it is easy to see how, under strategy $\str$, the set of states that are safe with probability $p$ increases for any $0<p<1$.  
  
%    \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{Stretegy10Steps.jpg}
%\caption{Syntesized strategy after $10$ disscrete steps. The action to apply at the next step depends on the particular state of the system. If the system is in the yellow region, then apply action $1$, otherwise apply action $2$. }
%\label{Figure:ExperimentStrategy10steps}
%\end{figure}%

 

%\begin{tabular}{|l|l|l|l|l|}\hline
%Numb Modes&dx & h  & Space Discr & Time Discr  \\
%\hline
% $1$ & $0.64$ & $0.1$   & $35$ sec & $45$ sec  \\
%  $1$ & $0.5$ & $0.1$  & $123$ sec & $47$ sec  \\
% $1$ & $0.4$ & $0.1$   & $373$ sec & $70$ sec  \\
% $1$ & $0.32$ & $0.1$   & $872$ sec & $107$ sec  \\
% $1$ & $0.2$ & $0.1$   & $21100$ sec & $377$ sec  \\
%  $2$ & $0.5$ & $0.1$   & $-$ sec & $-$ sec  \\
%\hline
%\end{tabular}

==> sections/time_discretization.tex <==
% time discretization


%\begin{figure}
%	\centering
%	\includegraphics[scale=0.25]{KernelCont.jpg} 
%	\caption{For a safe set $\safeSet$ the figure shows two paths. The one in bold is safe at the sampling time, and thus, it is safe according to a dicrete time model, but such a path is not safe considering a continuous time model. In fact, there exists a sampling interval where the path reaches the unsafe region.  }
%	\label{fig:timePaths}
%\end{figure}


% \begin{figure}
%	\centering
%\begin{subfigure}{.2\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{SyntesisNormal.jpg}
%     \caption{}
%     \label{{fig:timePaths}}
%   \end{subfigure}%
%\begin{subfigure}{.35\textwidth}
%  \centering
%  \includegraphics[width=1\linewidth]{SyntesisHybrid.jpg}
%  \caption{}
%  \label{fig:HybridSystem}
%\end{subfigure}
%\caption{Bla Bla BLA}
%   \end{figure} 
    
Here, we derive bounds for the quantities 
\begin{equation}
    \label{timeDiscrBoundsMaxGenw}
    \min_{x_1\in q_i}\contKernel(\h \mid x_1,q_j,a),\quad \max_{x_1\in q_i}\contKernel(\h \mid x_1,q_j,a).
\end{equation}
To this end, we first need to introduce the notion of bridge of a stochastic process \cite{chen2016stochastic}. 
Intuitively, the \textit{bridge} of a stochastic process is also a stochastic process for which both initial and final states are known.
Formally, for $\pX(t)$ with given initial and final states $x_1,x_2 \in \mathbb{R}^{m}$, fixed action $a\in \Aimdp$, and duration $\h \in \mathbb{R}_{\geq 0}$, the bridge $\bridge_{\pX}^{x_1,x_2,a,\h}(t)$ (or simply $\bridge_{\pX}(t)$ if the context is clear) is defined as
% \begin{multline*}
%     \bridge_{\pX}^{x_1,x_2,a,\h}(t)= \Big(\pX(t) \mid \pX(0)=x_1, \pX(\h)=x_2,\\
%     \forall t \in [0,\h], \pA(t) =a \Big).
% \end{multline*} 
\begin{eqnarray*}
    &\bridge_{\pX}^{x_1,x_2,a,\h}(t)= \pX(t), \quad \text { conditioned on }& \\
    &\pX(0)=x_1, \quad \pX(\h)=x_2, \quad \pA(t) =a \;\;  \forall t \in [0,\h].&
\end{eqnarray*} 
% Since $\pX(t)$ a Gaussian process, $\bridge_{\pX}$ is also Gaussian \cite{chen2016stochastic,sottinen2014generalized}.  % and referred to as a \emph{Gaussian bridge} \cite{chen2016stochastic,sottinen2014generalized}.
The following proposition guarantees that $\bridge_{\pX}(t)$ is a Gaussian process and derives its expectation and covariance from those of $\pX$ \cite{chen2016stochastic,sottinen2014generalized}.
\begin{proposition}[Proposition 4 in %\cite{sottinen2014generalized}]
\cite{gasbarra2007gaussian}]
    Let $\pX$ be the stochastic process described by \eqref{eq:switched-dynamics}. For $a\in \U,$ $x_1,x_2 \in \mathbb{R}^m$, $\bridge_{\pX}^{x_1,x_2,a,\h}$ is a Gaussian process $\bridge_\pX(t) \sim \N(E_{\bridge_{\pX}}(t), \cov_{\bridge_{\pX}}(t) )$ with the following expectation and covariance 
    \begin{align}
        E_{\bridge_\pX}(t) &= \cov_\pX(\h,t){\cov_{\pX}(\h)^{-1}}\big(x_2-E_{\pX}(\h)\big) \hspace{10mm} \nonumber \\ 
        &  \hspace{50mm} + E_{\pX}(t), \label{ExpBridge}\\
        % &E_{\bridge_\pX}(t) = \cov_\pX(\h,t){\cov_{\pX}(\h)^{-1}}\big(x_2-E_{\pX}(\h)\big) + E_{\pX}(t), \label{ExpBridge}\\
        \cov_{\bridge_{\pX}}(t) &= \cov_{\pX}(t)- \cov_{\pX}(\h,t)\cov_{\pX}(\h)^{-1} \nonumber \\
        &  \hspace{45mm} \cov_{\pX}(\h,t), \label{VarBridge}
        % &\cov_{\bridge_{\pX}}(t) = \cov_{\pX}(t)- \cov_{\pX}(\h,t)\cov_{\pX}(\h)^{-1} \cov_{\pX}(\h,t), \label{VarBridge}
    \end{align}
    where $\cov_\pX(t_1,t_2)$ is the covariance of process $\pX$ at times $t_1$ and $t_2$ given by
    \begin{align}
     	\cov_{\pX}(t_1,t_2) &= E \Big[ \big(\pX(t_1) - E_\pX(t_1) \big)  \big(\pX(t_2) - E_\pX(t_2) \big)^T \Big] \nonumber \\
      &= e^{F(a)t_2} \cov_{\pX}(0) (e^{F(a)t_1})^T + \nonumber \\
     	& \hspace{12mm} \int_{0}^{\min(t_1,t_2)} e^{F(a)(t_2-u)} G(a) G(a)^T  \nonumber \\
        & \hspace{35mm} (e^{F(a)(t_1-u)})^T du. \label{GaussianCoVariance}
        % &= e^{F(a)t_2} \cov_{\pX}(0) \big(e^{F(a)t_1}\big)^T + \nonumber \\
        % & \hspace{32mm} \cov_\pX(\min(t_1,t_2)). \label{GaussianCoVariance}
     \end{align}
\end{proposition}
\noindent
% $E_{\pX}[0]$ is the expectation of ${\pX}(0),$ and $Cov_{\pX}(0)$ is the covariance matrix of ${\pX}(0)$.
% \begin{proof}
%     $\pX$ is the solution of a linear SDE. Thus, it is a Gaussian process with expectation and variance given by \eqref{ExpectationSHS} and \eqref{VarianceSHS} \cite{arnold1974stochastic,sarkka2006recursive}. Being $\pX$ a Gausian process, its bridge ,$\bridge_{\pX},$ is still a Gaussian process \cite{gasbarra2007gaussian,sottinen2014generalized}. Thus, $\bridge_{\pX}$ is completely characterized by expectation and covariances, which are given by \eqref{ExpBridge} and \eqref{VarBridge}
% \end{proof}

\noindent
Process $\bridge_{\pX}$ describes the evolution of $\pX$ during $[0,\h]$ given that ${\pX}(0)$ and ${\pX}(\h)$ are known. 
% Importantly, $\bridge_{\pX}$ is still a Gaussian process.  
Since $\bridge_{\pX}$ is Gaussian, we can use the theory of Gaussian processes to derive bounds for $\contKernel(\h|x_1,q_j,a)$. 
Theorem \ref{UpperBoundTime} focuses on the upper bound.
\begin{theorem}
\label{UpperBoundTime}
    For polytopic regions $q_i,q_j \subseteq \safeSet$, it holds that
    \begin{equation}
        \label{eq:contkernel_max}
        \max_{x_1\in q_i} \contKernel(\h \mid x_1,q_j,a) \; \leq \; \max_{\bar{x}\in \bar{q}} \int_{ \safeSet} \hspace{-5mm} \N(z \mid \bar{x}, \cov_{\bridge_{\pX}} (\frac{\h}{2}) )dz,
    \end{equation}
    where %$C=\cov_{\bridge_{\pX}}(\frac{\h}{2})$, 
    % $\bar{q} = \Post(q_i|A_1) \oplus   \Post(q_j|A_2)$,
    % $\oplus$ is the Minkowski, and 
    \begin{eqnarray*}
        \bar{q} &=& \Post(q_i|A_1) \oplus \Post(q_j|A_2), \\
        A_1 &=& e^{F(a)\frac{\h}{2}} - \cov_{\pX}(\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1} \, e^{F(a) \h},\\
        A_2 &=& \cov_{\pX}(\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1},
    \end{eqnarray*} 
    and $\oplus$ is the Minkowski sum.
\end{theorem}
\begin{proof}
    Let $\mathcal{D}=\{t_1,t_2, \ldots\} \subset [0,\h]$ be a countable and dense subset of $[0,\h]$  such that $\frac{\h}{2}\in \mathcal{D}.$
    The upper bound on the continuous kernel from region $q_i$ to $q_j$ is the maximum safety probability of the bridge over all the possible initial points in $q_i$ and final points in $q_j$:
    \begin{align*}
        % & \hspace{6mm} 
        \max_{x_1\in q_i}  \; \contKernel  & (\h \mid q_j,x_1,a) \\
        & = \max_{(x_1,x_2)\in (q_i.q_j)} \prob(\bridge_{\pX}(t)\in \safeSet, \, \forall t \in [0,\h]) \\
        &=  \max_{(x_1,x_2)\in (q_i.q_j)} \prob(\bridge_{\pX}(t_i)\in \safeSet, \, \forall t_i \in \mathcal{D}) \\
        &\leq \max_{(x_1,x_2)\in (q_i.q_j)} \prob(\bridge_{\pX}(\frac{\h}{2})\in \safeSet) \\
        &= \max_{(x_1,x_2)\in (q_i.q_j)} \int_{ \safeSet} \hspace{-4mm} \N \big(z | E_{\bridge_{\pX}}(\frac{\h}{2}), \cov_{\bridge_{\pX}}(\frac{\h}{2}) \big)dz,
    \end{align*}
    % Covariance $\cov_{\bridge_{\pX}}(\frac{\h}{2},\frac{\h}{2})$ does not depend on $x_1,x_2$ and  Thus, 
    where the first inequality is due to the continuity of all the sample paths of $\bridge_{\pX}$ in $[0,h]$ (Example $38.3$ in \cite{billingsley2008probability}).
    In the above optimization, the only term that depends on $x_1$ and $x_2$ is $E_{\bridge_{\pX}}(\frac{\h}{2})$.  By rearranging the terms in \eqref{ExpBridge}, we have
    \begin{align*}
         % E_{\bridge_\pX}(\frac{\h}{2}) &=& \cov_{\pX} (\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1} x_2 \; + \\ 
         % & &  \Big( e^{F(a)\frac{\h}{2}} - \cov_{\pX}(\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1} \\
         % & & \hspace{45mm} e^{F(a)\h} \Big) x_1.
         E_{\bridge_\pX}(\frac{\h}{2}) =& \Big( e^{F(a)\frac{\h}{2}} - \cov_{\pX}(\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1} e^{F(a)\h} \Big) \\
          &  x_1 \; + \; \Big( \cov_{\pX} (\h,\frac{\h}{2}) \, \cov_{\pX}(\h)^{-1} \Big) x_2.
    \end{align*}
    Therefore, $E_{\bridge_\pX}(\frac{\h}{2})$ is the sum of linear transformations of $x_1$ and $x_2$.  Since $x_1\in q_i$ and $x_2 \in q_j$, the above optimization can be defined as a maximization over all the points in the Minkowski sum of the linear transformations of $q_i$ and $q_j$.
\end{proof}

% \noindent
% It is worth noting that, as done in the previous section, to solve the optimization problem in Theorem \ref{UpperBoundTime} we can work in the transformed space induced by the transformation matrix $\transfMatrix_b$ such that $\cov_{\bridge}(\frac{\h}{2})$ becomes the identity matrix. Then, for the computation of the max value in Theorem \ref{UpperBoundTime}, a straightforward extension of Theorem \ref{th:SpaceDiscretizationKKTOnditions} can be used.  In this extended version, the point $y$ at which $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz=0$ needs to be considered instead of the center point in Condition 1. Condition 2 remains the same, and in Conditions 3, $\nabla f(y)$ needs to be replaced with $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz$. As we will show  in Proposition \ref{prop:tran_unsafe} below, even tough $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz$ may not be expressible in closed form,  we can always over-approximate $\Post(\safeSet|\transfMatrix_b)$ such that we obtain a closed form for the gradient.

Theorem \ref{UpperBoundTime} shows that the upper bound of $\contKernel$ is given by a constrained maximization (over a convex region $\bar q$) of the integral of a normal distribution over $\safeSet$.  An efficient method of computation for this maximization problem is similar to the one introduced in Section \ref{sec:space_disc}.  That is to solve the problem in the transformed space where $\cov_{\bridge_\pX}(\frac{\h}{2})$ is the identity matrix.  Then, through a grid discretization of the transformed $\safeSet$ (the discretization needs to be over-approximating if a precise representation is not possible), the integral of the normal distribution over $\safeSet$ can be expressed as a summation of closed-form functions, similar to \eqref{eq:err_function}.  Then, a straightforward extension of Theorem \ref{th:SpaceDiscretizationKKTOnditions} can be used to compute the $\max$ value of this summation.  For details, see Proposition \ref{prop:tran_unsafe} and the ensuing discussion. 

% as done in the previous section, to solve the optimization problem in Theorem \ref{UpperBoundTime} we can work in the transformed space induced by the transformation matrix $\transfMatrix_b$ such that $\cov_{\bridge}(\frac{\h}{2})$ becomes the identity matrix. Then, for the computation of the max value in Theorem \ref{UpperBoundTime}, a straightforward extension of Theorem \ref{th:SpaceDiscretizationKKTOnditions} can be used.  In this extended version, the point $y$ at which $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz=0$ needs to be considered instead of the center point in Condition 1. Condition 2 remains the same, and in Conditions 3, $\nabla f(y)$ needs to be replaced with $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz$. As we will show  in Proposition \ref{prop:tran_unsafe} below, even tough $\nabla \int_{\Post(\safeSet | \transfMatrix_b)}\mathcal{N}(z\mid y, Id)dz$ may not be expressible in closed form,  we can always over-approximate $\Post(\safeSet|\transfMatrix_b)$ such that we obtain a closed form for the gradient.
 

%Consequently, this . %shown in the proof of the Theorem \ref{KKTOnditions}. 
% \ll{Yes, we do use KKT conditions to solve this, but this upper bound does not really make a difference on the final results. So, I would not want to spend too much time on this...Maybe we could just give the theorem without commenting too much about how to characterise those points.} % which will give a finite set of possible solutions. %However, in practice, for $h$ relatively small,  the above probability will be very close to $1$. So, the apparently not tight bound $\max_{x\in q_i}\contKernel(\h|q_j,x_1,a)\leq 1$ is often surprisingly accurate.


% We now focus on the computation of  $\min_{x_1 \in q_i}\contKernel(\h \mid q_j,x_1,a)$. 
In order to derive the lower bound of $\contKernel(\h \mid q_j,x_1,a)$, we employ the $1-$norm distance of a point $x \in \reals^m$ to a set $X \subseteq \reals^{m}$, defined as
% To derive the lower bound of $\contKernel$, we employ the taxicab distance (also called Manatthan or $1-$norm distance) of a point $x \in \reals^m$ to a set $X \subseteq \reals^{m}$ defined as
% \begin{eqnarray*} 
%     \cabdis{x-X} &=& \min_{x' \in X} \cabdis{x-x'} \\
%     &=& \min_{x' \in X} \sum_{i=1}^m |x^{(i)} - x'^{(i)}|,
% \end{eqnarray*}
\begin{equation*} 
    \cabdis{x-X} = \min_{x' \in X} \cabdis{x-x'} = \min_{x' \in X} \sum_{i=1}^m |x^{(i)} - x'^{(i)}|,
\end{equation*}
where $x^{(i)}$ denotes the $i$-th component of vector $x$. % From the definition of $\bridge_{\pX}$, it holds that all the paths of $\bridge_{\pX}$ are continuous and if they reach the unsafe region during a sampling interval then, necessarily, from $q_i$ they must have first reached $\safeSet$ and then from $\safeSet$ they will have to go in $q_j$.
% Assume $\min_{x_1\in q_i}|x_1- \partial \safeSet|_1 \geq \min_{x_2\in q_2}|x_2- \partial \safeSet|_1$. Call $\epsilon_{q_i}=\min_{x_1\in q_i}|x_1- \partial \safeSet|_1$. Then, we can state the following inequality
Hence, the minimum distance from a region $q \subseteq \safeSet$ to the boundary of $\safeSet$ can be written as
\begin{equation*}
    \epsilon_q = \min_{x \in q} \cabdis{x - \partial \safeSet},
\end{equation*}
where $\partial \safeSet$ is the boundary of $\safeSet$.  Then, we can bound $\contKernel$ from below by
\begin{align}
   \hspace{-2mm}
   \min_{x_1 \in q_i} &  \contKernel(\h \mid x_1,q_j,a) \nonumber \\
   & \hspace{-5mm} = 1 - \hspace{-4mm} \max_{(x_1,x_2) \in (q_i,q_j)} \hspace{-3mm} \prob( \exists t \in [0,\h] \text{ s.t. } \bridge_\pX(t) \notin \safeSet) \nonumber \\
   & \hspace{-5mm} \geq 1 - \hspace{-4mm} \max_{(x_1,x_2) \in (q_i,q_j)}  \hspace{-3mm} \prob \big( \exists t \in [0,\h] \text{ s.t. } \cabdis{\bridge_{\pX}(t) -x_1} \geq \epsilon_{q_i} \nonumber \\
   & \hspace{33mm}  \, \wedge \, \cabdis{\bridge_{\pX}(t) - x_2} \geq \epsilon_{q_j} \big).
   \label{BoundsTIme:TravelPath}
\end{align}
% Measurability of the above events is guaranteed by the continuity of the sample paths of $\pX$ \cite{billingsley2008probability}. %{\color{blue}Remember to have this in the implementation. THis allows us to have bounds that are directionals, and much better.}
%However, in general, there exists a non-zero measure set of paths that travel more than $\bar\epsilon$ during the sampling time, but still remain within the safe set.
The inequality in  \eqref{BoundsTIme:TravelPath} holds because the set of paths of $\bridge_{\pX}$ that remain within a distance $\epsilon_{q_i}$ from $x_1$ or within a distance $\epsilon_{q_j}$ from $x_2$ is guaranteed to be safe during $[0,\h]$, and hence
% a subset of the paths that stay in $\safeSet$ during $[0,\h]$. 
the complement of this set contains all the paths that are not safe during $[0,\h]$.
% Note that this inequality holds even if we would consider $|\bridge_{\pX}(t) -x_2|_1>\epsilon_{q_j}$. However, being $q_j$ closer to $\safeSet$ by assumption, this would result in a more conservative bound.
% Being $\bridge_{\pX}$ a Gaussian process, we can then use the properties of Gaussian processes to bound Eqn \eqref{BoundsTIme:TravelPath}. This is done in Theorem \ref{LowBOundDiscretization} below. 
Theorem \ref{LowBOundDiscretization} (below) shows how to compute a bound on \eqref{BoundsTIme:TravelPath}, but in order to arrive to this theorem, the following terms need to be defined first.


% Nevertheless, in order to formulate Theorem \ref{LowBOundDiscretization} we need to introduce the following terms.

For $i \in \{1,\ldots,m \}$, let $L_{\bridge^{(i)}}$ denote the maximum distance that the expectation of the $i$-th component of the bridge can travel.  Formally, 
% For $[0,\h]$ introduce the non-negative constant $L_{[0,\h]}$, which bounds the distance traveled by $E_{\bridge_{\pX}}$ and defined as
%{\color{red}MOdify this one, with the updated form of the constant.}
%\begin{align*}
% &E^{i,j}_{[0,h]}=-\inf_{(x_1,x_2,t)\in (q_i,q_j,[0,h])}\{\\
% &\quad \quad \quad\min \{|x_1-\partial \safeSet|_1,|x_2-\partial \safeSet|_1|\}- |E_{\bridge_{\pX}}(t)-\partial \safeSet|_1      \},\end{align*}
\begin{align*}
    L_{\bridge^{(i)}} = \sup_{(x_1,x_2,t_1,t_2)\in (q_i,q_j,[0,\h],[0,\h])} |{E_{\bridge^{(i)}_{\pX}}(t_1)-E_{\bridge^{(i)}_{\pX}}(t_2)}|,
\end{align*}
where $\bridge^{(i)}_{\pX}$ is the $i$-th component of $\bridge_{\pX}$, $E_{\bridge_{\pX}}(0)=x_1$, and $E_{\bridge_{\pX}}(\h)=x_2.$
%s term, due to fact that Gaussian processes are closed with respect to linear operations, allows us to center our Gaussian process to the closest point that $E_{\bridge_{\pX}}$ gets to the boundary during $[0,h]$. Consequently, in computing our bounds we can safely assume $\bridge_{\pX}$ is zero-mean. 
For $i\in \{1,...m \},$ let $\bar{\bridge}_{\pX}^{(i)}(t)$ be the zero-mean Gaussian process  
    $$\bar{\bridge}_{\pX}^{(i)}(t)= \bridge_{\pX}^{(i)}(t)-E_{\bridge_{\pX}^{(i)}}(t) .$$
%where $\bridge_{\pX}^{(i)}$ is the $i$-th component of $\bridge_{\pX}$.  
Intuitively, $\bar{\bridge}_{\pX}^{(i)}(t)$ represents 
% the distribution of the $i$-th component of the bridge by setting its mean to zero.
the $i$-th component of the bridge with zero mean.
Furthermore, for $i \in \{1,\ldots,m\}$, we use $K^{d,i}_{\bridge}>0$ to denote the constant that bounds the expected maximum variation of the process $\bar{\bridge}_{\pX}^{(i)}(t)$.  That is,
%     $$K_d^{\bridge}= \max_{i \in \{1,...,m\}} K_{d,i},$$
% where
%      $$\sup_{t_1,t_2 \in [0,\h]}(d_{i}(t_1,t_2))\leq K_{d,i} \h,$$
     $$ \sup_{t_1,t_2 \in [0,\h]} d_{i}(t_1,t_2) \leq K^{d,i}_{\bridge} \, \h,$$
where 
\begin{equation*}
    d_i(t_1,t_2)= \sqrt{E \Big[ \big( \bar{\bridge}_{\pX}^{(i)}(t_1)-\bar{\bridge}_{\pX}^{(i)}(t_2) \big)^2 \Big] } \;.
\end{equation*}
We can now state the following theorem, which shows how to bound the inequality in \eqref{BoundsTIme:TravelPath}.
\begin{theorem}
\label{LowBOundDiscretization}
    For regions $q_i,q_j \subseteq \safeSet$, $i \in \{1,\ldots,m \}$, let
    \begin{equation*}
        \eta_i = \frac{\epsilon^* }{m} -\big( L_{\bridge^{(i)}} + 12 \int_{0}^{\frac{1}{2}K^{d,i}_{\bridge} \h} \ln \left( \frac{2 K^{d,i}_{\bridge} \, \h}{ z} + 1 \right)^\frac{1}{2} d z\big),
    \end{equation*}
    where $\epsilon^* = \max \set{\epsilon_{q_i},\epsilon_{q_j}}$.
    % $\bar{\epsilon} = \epsilon_{q_i}-L$ assume 
   Assume $\eta_i > 0, \forall i \in \{1,...,m\}$. Then, it holds that
    \begin{equation*}
        % \min_{x_1 \in q_i}\contKernel(\h\mid &q_j,x_1,a)\geq \\
        % &1-2 \exp^{-\frac{\left(\epsilon_{q_i} - L - 12 \int_{0}^{\frac{K_d^{\bridge} \h}{2}}\sqrt{\frac{ K_{d}^{\bridge}\h}{2 x}}\ d x  \right)^2}{2\sigma_I^2}},
        \min_{x_1 \in q_i} \contKernel(\h \mid x_1,q_j,a) \geq 
        1 - 2 \sum_{i=1}^{m}\, e^{ -\frac{\eta_i^2}{2 \xi_i }},
    \end{equation*}
    where $\xi_i = \sup_{t\in [0,\h]} \cov_{\bar{\bridge}_{\pX}^{(i)}} (t)$.
\end{theorem}
\noindent
The proof of Theorem \ref{LowBOundDiscretization} is given in Appendix \ref{sec:proof_theorem_LowBOundDiscretization}.  It makes use of the Borell-TIS inequality \cite{adler2010geometry} and of Dudley's theorem \cite{dudley1967sizes} to bound \eqref{BoundsTIme:TravelPath}.
%Theorems \ref{UpperBoundTime} and \ref{LowBOundDiscretization} allow us to build an abstraction with an error that is local and changes for any pair of cells. This is particularly important because, intuitively, trajectories that start from the middle of the safe set are much more likely to remain safe during the sampling interval than those starting from the boundary of such set. 
%Both theorems are general and holds both for stable and unstable dynamics

Theorem \ref{LowBOundDiscretization} requires the computation of constant $L_{\bridge^{(i)}}$, which is always lower-bounded by 
\begin{equation*}
    L_{\bridge^{(i)}} \geq \max_{(x_1,x_2) \in (q_i,q_j)} |{x^{(i)}_1-x^{(i)}_2}|.  
\end{equation*}
For particular models, this bound can be tightened. For example, if $F$ and $G$ are diagonal matrices, $F$ is stable (i.e., all of its eigenvalues are negative), and $\safeSet$ is centered on the origin, then %if for all $k\in\{1,...,m \}$ and for all $(x_1,x_2)\in(q_i,q_j),$ $|x_{2,k}|\leq |x_{i,k}|,$
$L_{\bridge^{(i)}}=0$.  Intuitively, this is because $E_{\bridge_{\pX}}(t)$ always points towards the origin; hence, it is always moving away from the unsafe set.

The term $\eta_i$ in Theorem \ref{LowBOundDiscretization} is a constant, which represents the difference between the larger distance between $q_i$ or $q_j$ and the boundary of $\safeSet$, scaled by $m$, and a term that bounds the expectation of the supremum of $\bridge_{\pX}^{(i)}$ (loosely speaking, it is the maximum distance that the system can travel in the duration of $\h$ in expectation) given by the Dudley's entropy integral \cite{adler2010geometry}.  
% In order for the bound to make sense, we require $\eta>0$. 
There are two scenarios when $\eta_i$ can be non-positive: (i) both $q_i$ and $q_j$ are very close to the boundary, and (ii) $q_i$ and $q_j$ are far from each other.  In either case, we set the lower bound of $\contKernel$ to zero.
Intuitively, when both $q_i$ and $q_j$ are very close to the boundary, the chances that $\bridge_{\pX}^{(i)}$ for all $i$ remains safe are very low.  When $q_i$ and $q_j$ are far from each other, the lower bound of the transition probability between them is close to zero for small $\h$. 


% . However, in this case, the probability that during $[0,\h]$ $\pX$ will travel from $q_i$ and $q_j$ will be negligible for $\h$ small enough. Therefore, making this second scenario not influent for the final error.   

%\section{Time Discretization Backup}
% Call $$d_{min}=\min_{x \in q_i} |(x-(\partial S)_j)|_1$$
%and
%%$$d_{min}^j=\min_{x \in q_i} |(x_2-(\partial S)_j)|$$
%$$d_{max}=\min_{x \in q_i}\max_{j \in \{1,...n \}} |(x_2-\partial S_j)|$$
%and $x_{min}\in q_i$ the point the respective point, where $ |(x_2-\partial S_j)|${\color{red} Don't like this definition} is the euclidean distance between the $j-th$ component of $x$ and the safe set. 
%For $x_1,x_2 \in \mathbb{R}^{m},$ consider the following stochastic process   $$\bridge_{\pX}(t')=(X(t')|X(t)=x_1,X(t+h)=x_2,u=a),$$ which is defined for $t'\in [t,t+h]$. Being $X$ a Gaussian process during $[t,t+h]$, $\bridge_{\pX}$  is a Gaussian bridge \cite{gasbarra2007gaussian,sottinen2014generalized}.
%A Gaussian bridge is still a Gaussian process, whose covariance and mean functions can be derived as
%\begin{align}\label{VarBridge}
%&  E[\bridge_{\pX}(t)]={\cov_X(h,t)}{\cov_X(h)^{-1}}(\bar{x}-E[X(h)])+ E[X(t)]\\
%&  \cov_{\bridge_{\pX}}(t,s)= \cov_X(t,s) - {\cov_X(h,t)\cov_X(h)^{-1}\cov_X(h,s)}{}\label{VarBridge}
%\end{align}
%It is easy to see that $m$
%\begin{proposition}\label{BoundMaxTime2}
%If $d_{max}^{q_i,q_j}<max_{x\in q_i}|\partial S -x| $ then
%\begin{align*}
%\max_{x\in q_i}&\,\contKernel(\h|q_j,x_1,a)\leq\\
%&1-\max_{x\in q_i}(\int_{\safeSet} \mathcal{N}_{x}(E_{\bridge_{\pX}}(t+\frac{\h}{2}),{C}_{\bridge_{\pX}}(t+\frac{\h}{2}))dx),
%\end{align*}
%\end{proposition}


%\begin{proposition}\label{BoundMaxTime}
%If $d_{max}^{q_i,q_j}<max_{x\in q_i}|\partial S -x| $ then
%\begin{align*}
%\max_{x\in q_i}&\,\contKernel(\h|q_j,x_1,a)\leq\\
%&1-\min_{j\in [1,m]}(\int_{d_{min}^j+2 d_{max}+ K_e h} \mathcal{N}_{x}(0,{C}_{\bridge_{\pX}}^{j,j}(t+\frac{\h}{2}))dx),
%\end{align*}
%where ${C}_{\bridge_{\pX}}^{j,j}(t+\frac{\h}{2})$ is the j-th element of the diagonal of matrix ${C}_{\bridge_{\pX}}(t+\frac{\h}{2})$
%\end{proposition}
%\begin{proof}
%{\color{red}this proof is ok for the next proposition not this one. Need to use KKT conditions to maximize $q_i$}
%For any $t'\in [t,t+h]$ we have that
%\begin{align*}
%&\max_{x_1\in q_i,x_2\in q_j}\contKernel(t|x_2,x_1,a)\geq\\
%& \max_{x_1\in q_i,x_2\in q_j}Prob(\bridge_{\pX}(t')\in \safeSet)= \\
%&1-\min_{x_1\in q_i,x_2\in q_j}Prob(\bridge_{\pX}(t')\not\in \safeSet)\leq\\
%&1-\min_{x_1\in q_i,x_2\in q_j}Prob(|\bridge_{\pX}(t')-x_1|>|x_1-\partial \safeSet|)\leq\\
%&1-\min_{j\in [1,m]}\min_{x_1\in q_i,x_2\in q_j}Prob(|(\bridge_{\pX})_j(t')-x_{1,j}|>d_{min}^j\,)
%\end{align*}
%%For any $x_1,x_2,$ the random variable $(\bridge_{\pX})_j(t')-x_{1,j}$ has a normal distribution with mean
%%$E_{\bridge_{x_2}}(t') - x_{1,j} $ and variance 
% $ \cov_{\bridge_{\pX}}^{j,j}(t') .$ That is, the variance is independent of the discrete location.
%For $t_1,t_2 \in [t,t+h]$ it is easy to see that
%$$ |E_{\bridge_{\pX}}[t_1]-E_{\bridge_{\pX}}[t_2]|\leq 2 d_{max}+K_e h$$
%Due to the property of closure of normal distribution with respect to linear operations, this implies that for $j\in\{1,...,m \}$
%$$\int_{d_{min}}^{\infty} \mathcal{N}_x(E[\bridge_{\pX}])_j(t')]-x_{1,j},\cov_{\bridge_{\pX}}_j[t'])dx \geq$$ $$\int_{d_{min}+d_{max}+2K_e}^{\infty} \mathcal{N}_x(0,C[\bridge_{\pX}])_j(t'))dx. $$
%\begin{align*}
%    \min_{x_1\in q_i,x_2\in q_j}&Prob(|(\bridge_{\pX})_j(t')-x_{1,j}|>d_{min}\,)\geq\\
%    &\int_{d_{min}+d_{max}+2K_e}^{\infty} \mathcal{N}_x(0,\cov_{\bridge_{\pX}}^{j,j}(t'))dx.
%\end{align*}
%\end{proof}
%Proposition \ref{BoundMaxTime} allows us to bound $\max_{x\in q_i}\contKernel(\h|q_j,x_1,a)$ by simply computing a probability of a zero-mean univariate normal distribution, whose  variance can be computed from Eqn \eqref{Variance}.
%Such bound is sound because the variance of a switching diffusion is independent of the particular discrete location. As a consequence, we can simply reason over the components of the $X$, which during $[t,t+h]$, and for a fixed action, is a multivariate Gaussian process,  whose components then behave as univariate Gaussian processes.

%\begin{figure}
%\begin{center}
%\includegraphics[height=4cm]{jcaesar.eps}    % The printed column  
%\caption{Gaius Julius Caesar, 100--44 B.C.}  % wihh is 8.4 cm.
%\label{fig1}                                 % Size the figures 
%\end{center}                                 % accordingly.
%\end{figure}
%
% OR

%\begin{figure}
%\begin{center}
%\epsfig{file=jcaesar,wihh=7cm}
%\caption{Gaius Julius Caesar, 100--44 B.C.}
%\label{fig1}
%\end{center}
%\end{figure}
